Detecting and Diagnosing Incipient Building Faults Using Uncertainty Information from Deep Neural Networks

Early detection of incipient faults is of vital importance to reducing maintenance costs, saving energy, and enhancing occupant comfort in buildings. Popular supervised learning models such as deep neural networks are considered promising due to their ability to directly learn from labeled fault data; however, it is known that the performance of supervised learning approaches highly relies on the availability and quality of labeled training data. In Fault Detection and Diagnosis (FDD) applications, the lack of labeled incipient fault data has posed a major challenge to applying these supervised learning techniques to commercial buildings. To overcome this challenge, this paper proposes using Monte Carlo dropout (MC-dropout) to enhance the supervised learning pipeline, so that the resulting neural network is able to detect and diagnose unseen incipient fault examples. We also examine the proposed MC-dropout method on the RP-1043 dataset to demonstrate its effectiveness in indicating the most likely incipient fault types.

==> fdd.tex <==
\section{Background on Building FDD}
\label{sec:background}

\ac{FDD} helps reduce the operating and maintenance costs of a building, by ensuring the equipment works in proper conditions. If faults are captured in an early manner, prompt measures can be taken in time, before they become more severe and cause further economic losses~\cite{Chilton:1952}. Typical symptoms of building faults include abnormal system behaviors, excessive electricity demand, and inaccurate sensor measurement. Such abnormal conditions can be detected and diagnosed by constantly monitoring the system’s operation conditions, e.g. sensor readings; however, it is often not easy to detect these faults in practice, by just monitoring the major performance indices (e.g., IAQ and energy consumption). In fact, most building systems are designed in a way such that deviations in system operation are compensated for by some feedback mechanisms. For example, faulty valves and dampers in \acp{AHU} are difficult to identify since the increased cooling coil entering air temperature caused by a leaky hot water valve would be compensated for by increased mechanical cooling. An incorrect mixed air temperature due to excessive or inadequate outside air (damper fault) is usually compensated for by the increased cooling or heating load. If the faults have not reached certain severity levels, they could be left unnoticed for years. To identify these faults, especially those incipient ones, FDD strategies should be designed with capabilities to monitor not only the main performance indices, but also the various internal sensor readings collected during system operation. \red{Here, take a chiller fault as an example}

%In literature, building \ac{FDD} methods can be divided into three main categories, including model-based, signal-based, and data-driven methods~\cite{Dai2013from,Gao2015asurvey}. Model-based methods depend on explicit physical models of HVAC system at the device level, such as chillers, cooling towers, and air handling units (AHUs) \cite{Qin2005afault,Saththasivam2008predictive,Ru2008variable}. By capturing correlations between input and output parameters of physical models, model-based methods detect faults through evaluating parameter variations, such as residuals between sensor measurements and model predictions. However, physical models, to some extent, are not accurate and meticulous enough to  capture inner connections among different components due to errors and uncertainties. For example, authors of \cite{Dumidu2014mining} pointed out that model-based methods are not as practical as data-driven methods in terms of applying the FDD techniques to real buildings.}

In literature, building \ac{FDD} methods can be divided into three main categories, including model-based, signal-based, and data-driven methods~\cite{Dai2013from,Gao2015asurvey}. Model-based methods depend on explicit physical system models at the device level~\cite{Qin2005afault,Saththasivam2008predictive,Ru2008variable}. By capturing the correlations between the inputs and the output parameters of physical models, model-based methods detect faults through comparing between actual sensor measurements and model predictions. Because the model captures the underlying physical processes, it also helps diagnose the faults. Despite the advantages, it is often not easy to construct accurate physical models, especially for complicated systems like building \acp{CPS}, due to modeling errors and uncertainties. Authors of~\cite{Dumidu2014mining} pointed out that model-based methods are not as practical as data-driven methods in terms of applying the FDD techniques to real buildings.

%The signal-based methods mainly consider the correlations between faults and system output signals, where improved performance can be achieved by adding the signal of nominal status as a priority. Usually, the signal-based FDD focuses on electronic signals from sensor measurements of environmental parameters that indicate system states, such as the measurements of the vibrations of motors and rotary machines \cite{Dai2013from}. An example of signal-based FDD is \cite{Shun2014amodel}, which combined wavelet transformation with Principal Component Analysis (PCA) to diagnose faults in AHU. Nevertheless, due to the complexity of HVAC system, not all the measurements are suitable to be translated as system output signals that can be transferred to frequency domain from time domain.

Signal-based \ac{FDD} methods aim at finding signatures from sensor measurements that can be used to indicate faults. An example of signal-based FDD is~\cite{Shun2014amodel}, which combined wavelet transformation with \ac{PCA} to diagnose faults in AHU. Although such methods can achieve good performance in practice, it is a nontrivial task to extract relevant signals and signatures that can effectively indicate the faulty conditions. The complexity of building systems and the various types of faults therein add to the challenge of applying signal-based FDD methods to such systems.

By casting \ac{FDD} as a multiclass classification problem, many supervised learning approaches have demonstrated good results in telling different types of faults from normal conditions. These supervised machine learning methods include Multivariate Regression Models \cite{Mustafaraj:2010}, Bayes Classifiers~\cite{Hill:2007,Zhao:2013,Xiao:2014}, Neural Networks (NN)~\cite{Fan:2010,Zhu:2012,Du:2014}, Fisher Discriminant Analysis (FDA)~\cite{Du:2008}, Gaussion Mixture Model \cite{Jaikumar:2011}, Support Vector Data Description (SVDD)~\cite{Yang:2013,Zhao:2014}, and Support Vector Machines (SVM) \cite{Liang:2007,Han:2010,Chen:2011,Yan:2014,Mulumba:2015}. Recently,
Li~et.~al proposed a tree-structured learning method~\cite{li2016fault} that is not only able to recognize the fault types but also to determine serious the identified fault is; however, the method relies on well-labeled training data that indicates not only the fault type of each data point, but also its severity level (from $1$ to $4$). In real-world settings, it is often impractical to obtain such a comprehensive labeled dataset for supervised learning; in practice, \textit{labeled} data from fault-free and high-severity fault conditions are more easily accessible than from incipient, low-severity faults. On top of that, there are always \textit{unknown unknowns} that may come up as surprises to the \ac{FDD} algorithms; and desirably, the algorithms should be able to set alarms for such conditions. On the other hand, researchers have also explored unsupervised learning methods for \ac{FDD}, such as \ac{PCA}, \ac{SPC} and autoencoders. Depending only on positive (healthy) class data, such methods have found their use in detecting anomalies; however, they still lack the ability to diagnose these anomalies.

%\bjin{Soft faults can stay unattended for a long time before developing into more severe levels; it is often until then will the problems be addressed. false positive rates}

%Many supervised machine learning methods, such as Multivariate Regression Models \cite{Mustafaraj:2010}, Bayes Classifier \cite{Hill:2007,Zhao:2013,Xiao:2014}, Neural Networks (NN) \cite{Fan:2010,Zhu:2012,Du:2014}, Fisher Discriminant Analysis (FDA) \cite{Du:2008}, Gaussion Mixture Model \cite{Jaikumar:2011}, Support Vector Data Description (SVDD) \cite{Yang:2013,Zhao:2014}, and Support Vector Machines (SVM) \cite{Liang:2007,Han:2010,Chen:2011,Yan:2014,Mulumba:2015}, have demonstrated their effectiveness in settings with abundant and comprehensive training data. Li~et.~al recently proposed a tree-structured learning method~\cite{li2016fault} that is not only able to recognize the fault types but also to determine serious the identified fault is; however, the method depend on well-labeled training data that indicates not only the fault type of each data point, but also its severity level (from $1$ to $4$). In real-world settings, it is often impractical to obtain such a comprehensive labeled dataset for supervised learning; in practice, \textit{labeled} data from fault-free and high-severity fault conditions are more easily accessible than from incipient, low-severity faults. On top of that, there are always \textit{unknown unknowns} that may come up as surprises to the \ac{FDD} algorithms; and desirably, the algorithms should be able to set alarms for such conditions. On the other hand, researchers have also explored unsupervised learning methods for \ac{FDD}, such as \ac{PCA}, \ac{SPC} and autoencoders. Depending only on positive (healthy) class data, such methods have found their use in detecting anomalies; however, they lack the ability to diagnose these anomalies.

In this work, we attempt to extend the capability of supervised neural networks so that it can give useful uncertainty information that indicates its confidence about the prediction. The technique we employ is Monte Carlo dropout, which is to be introduced next.

%Research on \ac{FDD} generally classifies building faults into two categories: \textit{hard failures} that occur abruptly and cause the system to stop suddenly, and \textit{soft faults} that cause performance degradation but the system can still continue to function~\cite{Comstock2001}. While hard faults are dangerous and can cause heavy economic losses, they are generally more detectable with proper measurements and analysis. 

%\dan{A building fault means a deviation in the value of at least one characteristic variable from its normal expected behavior, including improper performances of HVAC systems, excessive building peak electrical demand, wrong system set-points and operation schedules, equipment malfunctions, inaccurate sensor measurements, and so on. By constantly monitoring system operations, FDD aims at detecting premature faults, diagnosing their causes and providing feedback to building operators, who can make prompt reaction before severe damage is added to the system or additional economic loss occurs~\cite{Chilton:1952}. Hence, advantages of building FDD including prolonging equipment life, improving the indoor comfort level, reducing the building operating costs and maintenance expenses, and so on~\cite{YangZhao:2013}. As mentioned in Section~\ref{sec:introduction}, most soft faults can hardly be reflected by immediate changes in IAQ and energy consumption. \textit{For example, faulty valves and dampers in air handling unit (AHU) are difficult to identify since the increased cooling coil entering air temperature caused by a leaky hot water valve would be compensated for by the increased mechanical cooling. An incorrect mixed air temperature due to excessive or inadequate outside air (damper fault) is usually compensated for by the increased cooling or heating load. Under those situations, faults could be unnoticed for years since the indoor air quality (IAQ) is generally not affected. To identify them, FDD strategies should be designed with capabilities to monitor the inner connections among different components.}}
